Scalable Thompson Sampling using Sparse Gaussian Process Models

Thompson Sampling (TS) from Gaussian Process (GP) models is a powerful tool for the optimization of black-box functions. Although TS enjoys strong theoretical guarantees and convincing empirical performance, it incurs a large computational overhead that scales polynomially with the optimization budget. Recently, scalable TS methods based on sparse GP models have been proposed to increase the scope of TS, enabling its application to problems that are sufficiently multi-modal, noisy or combinatorial to require more than a few hundred evaluations to be solved. However, the approximation error introduced by sparse GPs invalidates all existing regret bounds. In this work, we perform a theoretical and empirical analysis of scalable TS. We provide theoretical guarantees and show that the drastic reduction in computational complexity of scalable TS can be enjoyed without loss in the regret performance over the standard TS. These conceptual claims are validated for practical implementations of scalable TS on synthetic benchmarks and as part of a real-world high-throughput molecular design task.

==> old versions/Preliminaries_old.tex <==
\section{Problem Formulation}\label{Sec:PF}

We consider the sequential optimization of an unknown function $f$ over a compact set $\X\subset \Rr^d$. A sequential learning policy selects a batch of $B$ observation points $\{x_{t,b}\}_{b\in [B]}$ at each time step $t=1,2,\dots$ and receives the corresponding real-valued and noisy rewards $\{y_{t,b}=f(x_{t,b})+\epsilon_{t,b}\}_{b\in[B]}$, where $\epsilon_{t,b}$ denotes observation noise. Throughout this paper we use $[B]$ to denote $[B]=\{1,2,\dots,B\}$. 

As is common in both the bandits and GP literature, our analysis begins with the following sub-Gaussianity Assumption~\ref{AssNoise},  a direct consequence of which is that $\E[\epsilon_{t,b}] = 0$, for all~$t,b\in \Nn$.

\begin{assumption}\label{AssNoise}
We assume that $\epsilon_{t,b}$ are i.i.d., over both $t$ and $b$, $R-$sub-Gaussian random variables, where $R>0$ is a fixed constant. Specifically, 
$
\E[e^{h\epsilon_{t,b}}]\le \exp(\frac{h^2R^2}{2}),~\forall h\in \Rr, \forall t,b\in \Nn. 
$

\end{assumption}

Let $x^*\in\argmax_{x\in\X}f(x)$ be an optimal point.
% (assuming it is achievable and unique). 
We can then measure the performance of a sequential optimizer as its \emph{strict regret}, defined as the cumulative loss compared to $f(x^*)$ over a time horizon $T$
\begin{eqnarray} \label{eq:regdef}
R(T,B;f) = \E\left[\sum_{t=1}^T \sum_{b=1}^B f(x^*) - f(x_{t,b})\right],
\end{eqnarray}
where the expectation is with respect to the possible stochasticity in the sequence of the selected batch observation points $\{x_{t,b}\}_{t\in[T], b\in [B]}$. 
%For $t\ge1$ and the $\sigma-$algebras $ \mathcal{F}_{t}=\sigma(x_1,x_2,....,x_{t,b}, \epsilon_1, \epsilon_2,...,\epsilon_{t-1})$, $x_{t,b}$ is $\mathcal{F}_{t}$ measurable and $\epsilon_{t,b}$ is $\mathcal{F}_{t+1}$ measurable. 
%It is infeasible to learn the global maxima of $f$ over a very large action space, from noisy observations, without any regularity assumption on $f$ and the noise. 
Note that our regret measure (\ref{eq:regdef}) is defined for the true unknown  $f$. In contrast, the popular alternative {Bayesian regret} \citep[e.g. see][]{Russo2018TutorialTS, kandasamy2018parallelised} averages over a prior distribution for $f$. As upper bounds on strict regret directly apply to the Bayesian regret (but not necessarily the reverse), our results are stronger than can be achieved with the technique of \cite{Russo2014} that equates TS's Bayesian regret with that of the well-studied upper confidence bound policy.


Following \cite{Chowdhury2017bandit,srinivas2010gaussian, Calandriello2019Adaptive}, we also assume a regularity condition on the objective function (Assumption \ref{AssNorm}). This condition is motivated by kernelized learning models and their associated reproducing kernel Hilbert spaces (RKHS). %Let $k:\X\times\X\rightarrow\Rr$ be a positive definite kernel. A Hilbert space $H_k$ of functions on $\X$ equipped with an inner product $\langle \cdot, \cdot \rangle_{H_k}$ is called an RKHS with reproducing kernel $k$ if $k(\cdot,x)\in H_k$, for all $x\in\X$, and $\langle f,k(\cdot,x)\rangle_{H_k} = f(x)$ (reproducing property) for all $x\in\X$ and $f\in H_k$. An RKHS is completely specified by its kernel function and vice-versa. The inner product induces the RKHS norm $||f||^2_{H_k} = \langle f,f\rangle_{H_k}$ that can be interpreted as a measure of the complexity of $f$.
\begin{assumption}\label{AssNorm}
We assume that the RKHS norm of the objective function is bounded: $||f||_{H_k}\le \Bc$ for some $\Bc>0$, and $k(x,x')\le 1$ for all $x,x'\in\X$.
\end{assumption}

%where a notable example is $\nu=\frac{1}{2}$ that is referred to as the \emph{exponential kernel}. 
%The SE kernel can also be interpreted as a special case of Mat{\'e}rn when $\nu\rightarrow\infty$. 



% For a detailed construction of RKHSs and more examples we refer to \citet{Kanagawa2018}. Here, we provide an intuitive explanation of our assumption for particular classes of kernels, namely Squared Exponential (SE) and Mat{\'e}rn, which are perhaps the most popular kernels in practice \citep[see e.g.][]{Rasmussen2006, Snoek2012practicalBO},
% \begin{equation}\nn
% k_{\text{SE}}(x,x') = \exp \left(-\frac{r^2}{2l^2} \right), \qquad
% k_{\text{Mat{\'e}rn}}(x,x') = \frac{1}{\Gamma(\nu)2^{\nu-1}}\left(\frac{\sqrt{2\nu}r}{l}\right)^{\nu}B_{\nu}\left(\frac{\sqrt{2\nu}r}{l}\right),
% \end{equation}
% where $r=||x-x'||$ is the Euclidean distance between $x$ and $x'$, $l >0$ is referred to as lengthscale, $\nu>0$ is referred to as the smoothness parameter and $B_\nu$ is the modified Bessel function of the second kind. Variation over parameter $\nu$ creates a rich family of kernels.
% %where a notable example is $\nu=\frac{1}{2}$ that is referred to as the \emph{exponential kernel}. 
% The SE kernel can also be interpreted as a special case of Mat{\'e}rn when $\nu\rightarrow\infty$. When $\nu=n+\frac{1}{2}$, $n \in \Nn\cup\{0\} $ the Mat{\'e}rn kernel can be expressed as the product of an exponential and a polynomial of order $n$. 

% The RKHS of Mat{\'e}rn is equivalent to a Sobolev space with parameter $\nu+\frac{d}{2}$~\citep{Teckentrup2019, Kanagawa2018}. This observation provides an intuitive interpretation for the norm of Mat{\'e}rn RKHS as proportional to the cumulative $L_2$ norm of the \emph{weak derivatives} of $f$ up to $\nu+\frac{d}{2}$ order. I.e., in the case of Mat{\'e}rn family, our assumption on the norm of $f$ translates to the existence of weak derivatives of $f$ up to $\nu+\frac{d}{2}$ order which can be understood as a versatile measure for the smoothness of $f$ controlled by $\nu$. In the case of SE kernel, our regularity assumption implies the existence of all weak derivatives of $f$. For the details on the definition of weak derivatives and Sobolev spaces see~\cite{Hunter2001Analysis}. 

\section{Gaussian Processes and Sparse Models}\label{Sec:GPs}

GPs are powerful non-parametric Bayesian models over the space of functions \citep{Rasmussen2006} with a distribution specified by a mean function $\mu(x)=\E[\hat{f}(x)]$ and a positive definite kernel (or covariance function) $k(x,x') = \E\left[(\hat{f}(x)-\mu(x))(\hat{f}(x')-\mu(x'))\right]$. 
We provide here a brief description of the classical GP model and two sparse variational alternatives.

\subsection{Exact Gaussian Process models}
Suppose that we have collected a set of location-observation tuples $\H_{t} = \{\Xb_{t},\yb_{t}\}$, where $\Xb_{t}$ is the $tB\times d$ matrix of locations with rows $[\Xb_{t}]_{(s-1)B+b} = x_{s,b}$ and  $\yb_{t}$ is the $tB$-dimensional vector of observations with elements $[\yb_{t}]_{(s-1)B+b}=y_{s,b}$ for all $s\in[t], b\in[B]$.
% (recall that $y_{s,b} = f(x_{s,b})+\epsilon_{s,b}$). 
Then, given Gaussian observation noise\footnote{The GP-TS methods use surrogate GP models and assume a Gaussian noise to obtain closed form posterior distributions applied to the optimization of $f$. 
This Bayesian approach is only for the purpose of algorithm design and does not affect our general agnostic assumptions on $f$ (being fixed and unknown, living in a RKHS) and $\epsilon_{t,b}$ (being sub-Gaussian). The notation $\hat{f}$ is used to distinguish the GP model from the fixed $f$. The assumed variance $\tau$ for the noise has an effect similar to the regularization parameter in kernel ridge regression \citep[see][for more details]{Kanagawa2018}.} $\epsilon_{t,b}\sim\Nc(0,\tau)$, the posterior of $\hat{f}$ 
given the set of past observations $\H_{t}$, is a also a GP with mean function
% $\mu_t(x) \triangleq \E[\hat{f}(x)|\H_{t}]$ and kernel function $k_t(\cdot,\cdot)\triangleq  \E[(\hat{f}(x)-\mu_t(x))(\hat{f}(x')-\mu_t(x'))|\H_{t}]$
$\mu_{t}(\cdot)$ and kernel function $k_t(\cdot,\cdot)$ 
specified as follows:
\begin{eqnarray}
\mu_t(x) =  k^{\TP}_{\Xb_t,x} (K_{\Xb_t,\Xb_t}+\tau \Ib)^{-1} \yb_{t}
%\\\label{GPt} 
\quad
k_{t}(x,x') =  k(x,x') -  k^{\TP}_{\Xb_t,x} (K_{\Xb_t,\Xb_t}+\tau \Ib)^{-1} k_{\Xb_t,x'}.\label{GPt}
% \sigma_{t}(\x) &=& k^{1/2}_t(\x,\x),
\end{eqnarray}
Here, we denote $k_{\Xb_t,x}$ as the $tB$ dimensional column vector with entries $[k_{\Xb_t,x}]_{(s-1)B+b}= k(x_{s,b},x)$, and $K_{\Xb_t,\Xb_t}$ is the ${tB}\times{tB}$ positive definite covariance matrix with entries $[K_{\Xb_t,\Xb_t}]_{(s-1)B+b,(s'-1)B+b'} = k(x_{s,b}, x_{s',b'})$. Although GP models enjoy closed-form posterior expressions, calculating the posterior variance  of $\hat{f}(x)$ requires an $O((tB)^3)$ matrix inversion and so we see that exact GPs are computationally demanding computational bottleneck for large values of $tB$. 

% \footnote{The distribution of the noise $\epsilon_t$ is unknown and our only assumption is that it is sub-Gaussian. Our use of a Gaussian likelihood is merely for the purpose of algorithm design and does not effect our assumptions on $\epsilon_t$. The assumed variance $\tau$ has an effect similar to the regularization parameter in kernel ridge regression~(see~\cite{Kanagawa2018}).}.


% Our Thompson sampling algorithms use GP priors for the objective function\footnote{The objective function $f$ is fixed an unknown and our only assumption is that it lives in an RKHS. Our use of GP models for Bayesian optimization is merely for the purpose of algorithm design and does not effect our assumptions on $f$. We use the notation $\hat{f}$ to distinguish the GP model from the fixed $f$.}. 


\subsection{Sparse Variational Gaussian Process Models with Inducing Points}\label{Sec:SVGP}

To overcome the cubic cost of exact GPs, SVGPs \citep{Titsias2009Variational,Hensman2013} instead approximate the GP posterior  $\Pr(\hat{f} | \yb_t)$ through a  set of \emph{inducing points} $\Zb_t = \{z_1,..., z_{m_t}\}$ (with $m_t << tB$). Conditioning on the \emph{inducing variables}
$\ub_t = \hat{f}(\Zb_t)$ (rather than the $tB$ observations $\yb_t$) and specifying a prior Gaussian density $q_{t}(\ub_t) = \Nc(\mb_t, \Sb_t)$, yields an approximate posterior distribution that, crucially, is still  
% $q_t(\hat{f}(\cdot)) = \int \Pr[\hat{f}(\cdot) | \ub_t] q_{t}(\ub_t) d\ub_t$. 
a GP but with the significantly reduced computational complexity of $O(tB m_t^2)$. The posterior mean and covariance of the SVGP is given in closed form as
\begin{eqnarray}\nn
{\mu}^{(s)}_t(x) = k_{\Zb_t,x}^{\TP} K^{-1}_{\Zb_t,\Zb_t}\mb_t\quad
{k}^{(s)}_t(x, x') = k(x,x')+ k_{\Zb_t,x}^{\TP}K^{-1}_{\Zb_t,\Zb_t} (\Sb_t - K_{\Zb_t,\Zb_t})K^{-1}_{\Zb_t,\Zb_t} k_{\Zb_t,x'}.\nn
\end{eqnarray}
The variational parameters $\mb_t$ and $\Sb_t$ are set as the maximizers of the evidence lower bound (ELBO, see appendix for details) and can derived explicitly for a conjugate likelihood \citep{Titsias2009Variational} (which is the case here) or optimized numerically with mini-batching \citep{Hensman2013}.


Although there are various standard ways in practice to select the locations of the inducing points $\Zb_t$, for the purpose of theoretical analysis, we make the same assumption as \cite{Burt2019Rates} and assume that $\Zb_t$ are sampled from $\Xb_t$ according to a discrete k-Determinantal Point Process (k-DPP). While sampling according to an exact k-DPP distribution might be costly, defying the computational gain of SVGP, \citeauthor{Burt2019Rates} showed that $\Zb_t$ can be efficiently sampled from \emph{$\epsilon_0$ close} sampling methods without compromising the predictive quality of SVGP. 






%\cite{Titsias2009Variational} provides an explicit solution for the convex optimization problem of finding $\mb_t, \Sb_t$. \citet{Hensman2013} proposed an efficient numerical solution allowing for mini-batching.  
% To optimize the ELBO in practice, \citet{Hensman2013} proposed a numerical solution allowing for mini-batching \citep[see also][]{Burt2019Rates} and the use of stochastic gradient descent algorithms, such as Adam~\citep{kingma2014adam}. In addition, \citet{Titsias2009Variational} provides an explicit solution for the convex optimization problem of finding $\mb_t, \Sb_t$ ), allowing more involved alternate optimization schemes.


% \begin{eqnarray}
% \Lc_{\text{lower}} = \frac{-1}{2}\yb^{\TP}Q^{-1}\yb -\frac{1}{2}\log |Q| - \frac{t}{2}\log(2\pi) -\frac{t}{2\tau}
% \end{eqnarray}
% A natural way of approximating posterior GPs is to represent $\hat{f}$ in terms of its behavior $\ub = \hat{f}(\Zb)$ at a carefully chosen set of \emph{inducing points} $\Zb = \{z_1,..., z_M\}$. \iffalse Rather than directly conditioning on observations $\yb$,\fi Sparse GPs specifies Gaussian density $q(\ub) = \Nc(\mb, \Sb)$ that explains the data. The posterior distribution is approximated as
% $p(\hat{f}| \yb) \approx q(f) = \Nc(\tilde{\mu}(\cdot), \tilde{\sigma}(\cdot))$
% where in case of GPs, $\ub\sim \Nc(\mu^{\ub}, \Sigma^{\ub})$. This results in the sparse approximation of posterior mean and covariance as
% \begin{eqnarray}\nn
% \tilde{\mu}(\cdot) &=& k_{\ub}^{\TP}(\cdot) K^{-1}_{\ub\ub}\mb\\
% \tilde{\sigma}(\cdot) &=& k(\cdot,\cdot) + k_{\ub}^{\TP}(\cdot)K^{-1}_{\ub\ub} (\Sb - K_{\ub\ub})K^{-1}_{\ub\ub} k_{\ub}(\cdot)
% \end{eqnarray}
% where the variational parameters $\mu^{\ub}$ and $\Sigma^{\ub}$ are the maximizer of the evidence lower bound and can be calculated efficiently~\citep{Titsias2009Variational, Burt2019Rates}. 
% \begin{eqnarray}
% \Lc_{\text{lower}} = \frac{-1}{2}\yb^{\TP}Q^{-1}\yb -\frac{1}{2}\log |Q| - \frac{t}{2}\log(2\pi) -\frac{t}{2\tau}
% \end{eqnarray}
% \sattar{details }






\subsection{Sparse Variational Gaussian Process Models with Inducing Features}\label{Subsec:feature}

An alternative approximation strategy for GPs with the same computational complexity as inducing point approximations but with sometimes improved accuracy are inducing feature approximations \citep{hensman2017variational,Burt2019Rates, dutordoir2020}. Here, we
% Rather than setting inducing variables $\ub_t$ as the random variables obtained when evaluating a set of inducing points, we could alternatively 
define inducing variables as the linear integral transform of $\hat{f}$ with respect to some \emph{inducing features} \citep{lazaro2009inter} $\psi_1(x),..,\psi_{m_t}(x)$, i.e  $u_{t,i} = \int_{\X} \hat{f}(x)\psi_i(x)dx$.  Courtesy of Mercer's theorem, we can decompose our chosen kernel $k$ as the inner product of possibly infinite dimensional feature maps (see Theorem 4.1 in~\citeauthor{ Kanagawa2018}) to provide the expansion $k(x,x') = \sum_{j=1}^{\infty}\lambda_j\phi_j(x),\phi_j(x')$ for eigenvalues $\{\lambda_j\in \Rr^+\}_{j=1}^{\infty}$ and eigenfunctions $\{\phi_j\in H_k\}_{j=1}^\infty$. If we set our inducing features to be the $m_t$ eigenfunctions with largest eigenvalues, it can be shown that  $\text{cov}(u_{t,i}, u_{t,j}) = \lambda_j \delta_{i,j}$ and $\text{cov}(u_{t,j}, \hat{f}(x)) = \lambda_j \phi_j(x)$ , yielding an approximate Gaussian Process model with  posterior mean and covariance given by
\begin{eqnarray}\nn
{\mu}^{(s)}_t(x) = \phib_{m_t}^{\TP}(x)\mb_t\qquad {k}^{(s)}_t(x,x') = k(x,x') +   \phib_{m_t}^{\TP}(x)(\Sb_t-\Lambda_{m_t})\phib_{m_t}(x').
\end{eqnarray}
Here, $\mb_t$ and $\Sb_t$ are inducing parameters (set to be maximizers of the ELBO),  $\phib_{m}(x)\triangleq [\phi_1(x),...,\phi_m(x)]^{\TP}$ is the truncated feature vector and $\Lambda_m$ is the $m\times m$ diagonal matrix of eigenvalues, $[\Lambda_m]_{i,j}=\lambda_i\delta_{i,j}$. 
% The expression of ELBO is the same as in \ref{eq:elbo}, with $Q_t = K^{\TP}_{\phib_{m_t},\Xb_t} \Lambda^{-1}_{m_t}K_{\phib_{m_t},\Xb_t}$, $K_{\phib_{m_t},\Xb_t} = [\lambda_i\phi_i(x_j)]_{i,j}$, $i=1,\dots, m_t$, $j=1,\dots,t$. 



==> old versions/introduction_vic.tex <==
\section{Introduction}\label{Intro}

Thompson sampling \citep[TS,][]{Thompson1933} is a popular algorithm for Bayesian optimization \citep[BO,][]{Shahriari2016} --- a sequential model-based approach for the optimization of expensive black-box functions, as characterised by limited prior knowledge and access to only a limited number of (possibly noisy) evaluations. By sequentially evaluating the maxima of random samples from our current model of the objective function, TS provides an conceptually simple method for balancing the exploration-exploitation trade-off that arises when optimizing under uncertainty. TS is often paired with Gaussian Processes \citep[GP,][]{Rasmussen2006}, a spectrum of powerful and flexible models that can be used to make predictions of the objective function. These GP-TS methods \citep{Chowdhury2017bandit} have been found very efficient in a small data scenario, with numerous successful applications  including aerodynamic design \citep{baptista2018bayesian}, route planning \citep{eriksson2021scalable} and web-streaming \citep{daulton2019thompson}. 



Most BO algorithms query one (or a handful of) observation(s) at a time and require a substantial amount of computational time between two queries,
as it updates GP models and search for the next point to query.
This makes BO particularly unfit for large data regimes. However, scaling up with the number of observations would expand its usability, in particular to 
highly noisy problems, rougher optimization landscape or higher dimension.
Among the many propositions to scaling up BO, one can mention using replicates and averaging, \citep[see e.g.][]{jalali2017comparison,binois2019replication},
using Neural Networks in lieu of GPs \citep{snoek2015scalable,hernandez2017parallel}, local \citep{eriksson2019scalable} or ensemble of models \citep{wang2018batched}.
One key advantage of TS is its natural ability to query large batches of points at a time \citep{hernandez2017parallel,kandasamy2018parallelised},
while most alternatives cannot scale beyond a couple of points \citep{chevalier2013fast,gonzalez2016batch,wu2016parallel,letham2019constrained,moss2021gibbon}.
With large batches, the computational cost of BO is considerably reduced, which makes GP-TS a great candidate for much larger data volumes.

However, the practical implementation of GP-TS introduces two main difficulties that prevent the method from scaling in terms of time horizon. 
First, building the GP posterior distribution, which is needed every time a new batch of observations is acquired, is well known to require an $O(t^3)$ computation (where $t$ is the number of observations) due to a matrix inversion step~\citep{Rasmussen2006}.
Given the updated posterior model, sampling from its optimum is the second challenging task. The standard approach is to draw a joint sample on a grid discretizing the search space. Sampling over a grid of size $N$ has an $O(N^3)$ complexity \citep[due to a Cholesky decomposition step,][]{diggle1998model}, which is the second computational bottleneck.

A natural answer to the first challenge is to rely on the recent advances in sparse variational GP models (referred to as SVGP for the rest of the paper), 
which allow a low rank approximation of the GP posterior in $O(m^2 t)$ computation, where $m$ is the number of the so-called \emph{inducing variables} and grows at a rate much slower than $t$~\citep{Titsias2009Variational}. 
The inducing variables are manifested either as \emph{inducing points} or \emph{inducing features} \citep[sometimes referred to as inducing inter-domain variables,][]{Burt2019Rates,vanderWilk2020Framework,dutordoir2020}.
Furthermore, \cite{wilson2020efficientsampling} introduced an efficient sampling rule (referred to as \emph{decoupled } sampling) which decomposes a sample from the posterior into the sum of a prior with $M$ features (see Sec.~\ref{Subsec:feature}) and an SVGP update, reducing the computational cost of drawing a sample to $O\left((m+M)N\right)$. Leveraging this sampling rule
results in a scalable GP-TS algorithm (henceforth S-GP-TS) that is simple to implement and can handle orders of magnitude larger number of observation points. 

In this work, we provide the first theoretical analysis of S-GP-TS, investigating whether this scalable approach  maintains the performance guarantees of TS over exact GPs (GP-TS). Unlike many algorithms used for BO, TS is motivated by a rich body of theoretical work, with a comprehensive analysis across the multi-armed bandits \citep{Kaufmann2012,Agrawal2013TS,Kaufmann2013TS,Gopalan2014TS,Russo2016Info,Abeille2017LinTS} and reinforcement learning [ADD REFS] literatures. Although this theory has been extended to BO for TS from exact GP models \citep{Chowdhury2017bandit}, it has yet to be expanded for scalable TS methods or for batch optimization. Indeed, using sparse models and decoupled sampling introduce two layers of approximation,
that must be handled with care, as even a small constant error in the posterior can lead to poor performance bu encouraging under-exploration in the vicinity of the optimum point \cite{Phan2019TSExample}. 

Our primary contributions can be summarised as follows:
% First, a theoretical analysis showing that batch TS from an approximate GP can achieve the same regret order as an exact GP-TS algorithm as long the quality of the posterior approximations satisfies certain conditions (Assumptions~\ref{Ass1} and~\ref{Ass2}). 
% Second, for the specific case of S-GP-TS (batch decoupled TS over an SVGP), we leverage the results of \cite{Burt2019Rates} to provide bounds in terms of GP's kernel spectrum for the number $M$ of prior features and the number $m$ of inducing variables required to guarantee low regret.
% Finally, we investigate empirically, the performance of multiple practical implementations of S-GP-TS, considering synthetic benchmarks and a real-world high-throughput molecular design task. 
\begin{itemize}
    \item A theoretical analysis showing that batch TS from any approximate GP can achieve the same regret order as an exact GP-TS algorithm as long the quality of the posterior approximations satisfies certain conditions (Assumptions~\ref{Ass1} and~\ref{Ass2}). 
    \item For the specific case of S-GP-TS (batch decoupled TS over an SVGP), we leverage the results of \cite{Burt2019Rates} to provide bounds in terms of GP's kernel spectrum for the number $M$ of prior features and the number $m$ of inducing variables required to guarantee low regret.
    \item We investigate empirically the performance of multiple practical implementations of S-GP-TS, considering synthetic benchmarks and a real-world high-throughput molecular design task. 
\end{itemize}



